Lower Bounds for the Graph Homomorphism Problem

The graph homomorphism problem (HOM) asks whether the vertices of a given $n$-vertex graph $G$ can be mapped to the vertices of a given $h$-vertex graph $H$ such that each edge of $G$ is mapped to an edge of $H$. The problem generalizes the graph coloring problem and at the same time can be viewed as a special case of the $2$-CSP problem. In this paper, we prove several lower bound for HOM under the Exponential Time Hypothesis (ETH) assumption. The main result is a lower bound $2^{\Omega\left( \frac{n \log h}{\log \log h}\right)}$. This rules out the existence of a single-exponential algorithm and shows that the trivial upper bound $2^{{\mathcal O}(n\log{h})}$ is almost asymptotically tight. We also investigate what properties of graphs $G$ and $H$ make it difficult to solve HOM$(G,H)$. An easy observation is that an ${\mathcal O}(h^n)$ upper bound can be improved to ${\mathcal O}(h^{\operatorname{vc}(G)})$ where $\operatorname{vc}(G)$ is the minimum size of a vertex cover of $G$. The second lower bound $h^{\Omega(\operatorname{vc}(G))}$ shows that the upper bound is asymptotically tight. As to the properties of the "right-hand side" graph $H$, it is known that HOM$(G,H)$ can be solved in time $(f(\Delta(H)))^n$ and $(f(\operatorname{tw}(H)))^n$ where $\Delta(H)$ is the maximum degree of $H$ and $\operatorname{tw}(H)$ is the treewidth of $H$. This gives single-exponential algorithms for graphs of bounded maximum degree or bounded treewidth. Since the chromatic number $\chi(H)$ does not exceed $\operatorname{tw}(H)$ and $\Delta(H)+1$, it is natural to ask whether similar upper bounds with respect to $\chi(H)$ can be obtained. We provide a negative answer to this question by establishing a lower bound $(f(\chi(H)))^n$ for any function $f$. We also observe that similar lower bounds can be obtained for locally injective homomorphisms.

==> lowerbounds.tex <==
\section{Lower bounds for the graph homomorphism problem}\label{sec:lowerbounds}
\begin{proof}[of Theorem~\ref{main:theorem_homs}]
\input{mainproof.tex}
\end{proof}

==> planarbound.tex <==
\subsection{Lower bounds for planar graphs}
The \textsc{Planar Graph Homomorphism} problem PHOM$(G,H)$ and the \emph{List Planar Graph Homomorphism} problem P-LIST-HOM$(G,H)$ are HOM and LIST-HOM problems where $G$ is restricted to be a planar graph. First, we note that the P-LIST-HOM$(G,H)$ problem can be solved in time $2^{\cO(\sqrt{n}\log{h})}$. Indeed, by the planar separator theorem~\cite{LT1979}, in any planar graph one can find a separator of size $\cO(\sqrt{n})$ such that each of disjoint subgraphs has at most $2n/3$ vertices. This immediately gives us a $2^{\cO(\sqrt{n}\log{h})}$ upper bound for the problem. In this section we show a lower bound $2^{\Omega(\sqrt{n\log{h}/\log\log{h}})}$ under the ETH assumption.

In this section we use the hardness of \textsc{$3$-Coloring} on planar graphs. We show a counterpart of Lemma~\ref{lemma:3col}, i.e., we show that this problem remains hard on graphs of bounded maximum degree.

\begin{proposition}[\cite{L1982} and Theorem~$9.9$ in~\cite{CFKLMPPS2014}]
Unless ETH fails, there exists a constant $\alpha>0$ such that  \textsc{$3$-Coloring} on $n$-vertex planar graphs cannot be solved in time $\cOs\left(2^{\alpha n^{1/2}} \right)$.
\end{proposition}

\begin{lemma}
\label{lem:3colp}
Unless ETH fails, there exists a constant $\beta >0$  such that there is no algorithm solving \textsc{$3$-Coloring} on $n$-vertex planar graphs of maximum degree five in time $\cOs\left(2^{\beta n^{1/2}} \right)$.
\end{lemma}
\begin{proof}
For a given $n$-vertex planar graph $G$, we construct a planar graph $G'$ with maximum vertex degree five and  $|V(G')|<18|V(G)|$ such that $G$ is $3$-colorable if and only if $G'$ is. Then we set $\beta=\alpha/\sqrt{18}>0$ which finishes the proof of Lemma.

Let $v$ be a vertex of a planar graph $G$ of degree $d>5$, let $u_1,\ldots,u_d$ be the neigbors of $v$. We replace $v$ with $d+2(d-1)$ vertices: $v_1,\ldots,v_d,a_1,\ldots,a_{d-1},b_1\ldots,b_{d-1}$. For all $1\le i\le d-1$, we add edges $\{v_i, a_i\}, \{a_i, b_i\}, \{b_i,v_i\}, \{v_i, u_i\}$. For all $2\le i\le d$, we add edges $\{v_i,a_{i-1}\}$ and $\{v_i,b_{i-1}\}$. Note that this ensures that all $v_i$'s are colored the same color. Now it is easy to see that a $3$-coloring of one graph implies a $3$-coloring of the other. Also note that we added at most $6|E(G)|<18|V(G)|$ vertices.
\end{proof}

\begin{theorem}\label{main:theorem_homs} 
Unless ETH fails, there exists a constant $c)>0$ such that
for any 
%non-decreasing time-constructible
function
$3\le h(n)\le 2^{o(n)}$,
there is no algorithm solving \textsc{Planar List HOM$(G,H)$} for an $n$-vertex graph $G$ and $h(n)$-vertex graph $H$ in time 
\begin{equation}\label{eq:planar}
\cOs\left(2^{c\left(\frac{n\log{h(n)}}{\log\log{h(n)}}\right)^{1/2}} \right) \,.
\end{equation}
\end{theorem}

\begin{proof}
Assuming the existence of an algorithm that solves \textsc{Planar List HOM$(G,H)$} in time~(\ref{eq:planar}) for $c=\beta/\sqrt{350}$, we show that \textsc{Planar $3$-coloring} can be solved in time $\cOs\left(2^{\beta n'^{1/2}} \right)$ on graphs of maximum degree five with $n'=nr/5$ vertices where $r=\frac{\log h(n)}{70\log\log h(n)}$. Since $h(n)$ is a non-decreasing function, this would solve \textsc{Planar $3$-coloring} for infinitely many values of $n$, that by Lemma~\ref{lem:3colp}, contradicts to ETH.

Let $G$ be a planar graph of maximum degree five with $n'=nr/5$ vertices that needs to be $3$-colored. Without loss of generality we assume that $G$ is a connected graph. Then we take any spanning tree $T$ of $G$. Since the maximum degree of $T$ is five, we can partition it into connected graphs $G_1,\ldots,G_k$, such that for all $1\le i\le k-1$, $r/4\le|V(G_i)|\le r$, $|V(G_k)|\le r$. Now we add at most $k\cdot r \le 4nr/5$ isolated vertices to make all the graphs $G_i$ have precisely $r$ vertices. Let $G'$ be the obtained graph with at most $nr$ vertices, and $G_i$ for $1\le i\le k$ be buckets of its edge-preserving $r$-grouping. Since the planar graphs are closed under taking minors, the obtained edge-preserving $r$-grouping of $G'$ is a planar graph with at most $n$ vertices. 

Now we use Lemma~\ref{lemma:3coltolisthom} with $r=\frac{\log h(n)}{70\log\log h(n)}$ and this specific edge-preserving $r$-grouping of $G'$, to get an equisatisfiable instance $(G'',H'')$ of LIST-HOM with $|V(G'')|\le n$ and $|V(H'')| \le r^{70 r}$. Note that $V(H'')| \le r^{70 r}=2^{\frac{70\log h(n) (\log\log h(n) - \log70 - \log\log\log h(n))}{70\log\log h(n)}}<2^{\frac{70\log h(n) (\log\log h(n))}{70\log\log h(n)}}=h(n)$. 
Thus, an algorithm with running time \eqref{eq:planar} for \textsc{Planar List HOM} implies an algorithm for \textsc{Planar $3$-coloring} with running  time
\[
\cOs\left(2^{c\left(\frac{n\log{h(n)}}{\log\log{h(n)}}\right)^{1/2}} \right)=
\cOs\left(2^{c\left(n70r\right)^{1/2}} \right)=\cOs\left(2^{c\left(350n'\right)^{1/2}} \right)=\cOs\left(2^{\beta n'^{1/2}} \right).
 \]
\end{proof}

%Informally, the idea is as follows. Denote by $(n, \Delta, d)$-PHOM problem
%the (directed) homomorphism problem where $n$ is the number of vertices of
%the left \emph{planar} graph, $\Delta$ is a strict upper bound on its maximal degree, and $d$ is the number of vertices
%of the right graph. The main ingredient of the proof is the following reduction:
%\[ (n, \Delta, d) \to (n/2, 2\Delta, 4\Delta^2d^22^{16\Delta^2}) \, .\]
%That is, given an instance of PHOM with the left graph having $n$ vertices and degree $\Delta$ one can construct (in polynomial time) an equisatisfiable instance
%with $n/2$ vertices and degree $2\Delta$. Now, from Lemma~\ref{thm:3colp} we know that there exist $\Delta_0, d_0 = O(1)$ such that there are no $c^{\sqrt{n}}$ algorithm for $(n, \Delta_0, d_0)$-PHOM. Using the reduction above we can transfer the lower bound
%to any large $d$.
%
%\begin{lemma}
%\label{lemma:red}
%Given an instance of $(n, \Delta, d)$-LIST-PHOM one can construct in polynomial time
%an equisatisfiable instance of $(n/2, 2\Delta, 4\Delta^2d^22^{16\Delta^2})$-LIST-PHOM.
%\end{lemma}
%\begin{proof}
%Let $G$ be a graph on $n$ vertices with maximal degree less than $\Delta$
%and $H$ be a graph on $d$ vertices. For each vertex of $G$ we are also given a list
%of allowed vertices from $H$.
%
%The graph $G'$ is obtained from $G$ by contracting pairs of vertices.
%Namely, let $V(G)=[n]$. Then $V(G')=\{(1,2), (3,4), \ldots, (n-1,n)\}$.
%Vertices $(i,j)$ and $(k,l)$ are joined by an edge in $G'$ iff
%some of $i$ and $j$ is connected with some of $j$ and $k$ in $G$.
%Clearly, the number of vertices in $G'$ is $n/2$ and its degree is less than $2\Delta$.
%As in Theorem~\ref{thm:glhtocsp}, one can color $G'$ in $4\Delta^2$ 
%colors such that all the neighbors of any vertex have different colors.
%Denote the set of all colors by~$C$.
%
%Vertices of the graph $H'$ are given by quadruples $(c,d_0,d_1,g)$ where
%$c \in C$, $d_0, d_1 \in H$, and $g \colon C \times \{0,1\}^2 \to \{0,1\}$.
%Thus, the number of vertices in $H'$ is $4\Delta^2d^22^{16\Delta^2}$.
%Two vertices $(c,d_0,d_1,g)$ and $(c',d_0',d_1',g')$ are joined by an edge
%in $H'$ iff for all $i,j \in \{0,1\}$, $g(c,i,j)\le[(d_i,d_j') \in H]$.
%
%Finally, for each vertex $(i,j) \in V(G')$ we give a list of allowed vertices from $H'$.
%A vertex $(c, d_0, d_1, g) \in V(H')$ is allowed for $(i,j) \in V(G')$ iff
%\begin{enumerate}
%\item $\operatorname{color}(i,j)$ is $c$;
%\item if $(i,j) \in E(G)$ then $(d_0,d_1) \in E(H)$;
%\item $i \in V(G)$ is allowed to be mapped to $d_0 \in V(H)$
%and $j \in V(G)$ is allowed to be mapped to $d_1 \in V(H)$;
%\item for any neighbour $(k,l)$ of $(i,j)$ in $G'$, the four bits of $g(\operatorname{color}(k,l))$ are consistent with the edges between
%$i,j$ and $k,l$ in $G$.
%\end{enumerate}
%
%It is easy to see that the initial and the constructed instances are equisatisfiable.
%\end{proof}
%
%\begin{theorem}
%Under the ETH assumption there exists a constant $\gamma$ such that
%\begin{enumerate}
%\item There is no $2^{\sqrt{n} \log^{\gamma} d}$ algorithm for $(n,d)$-PHOM.
%\item For $d=O(1)$, there is no $2^{\sqrt{n} \log^{\gamma}d}f(d)$ algorithm for $(n,d)$-PHOM.
%\end{enumerate}
%\end{theorem}
%\begin{proof}
%Lemma~\ref{thm:3colp} implies that there exist 
%$\Delta_0, d_0 = O(1)$ such that there is no $c_0^{\sqrt{n}}$ algorithm for $(n, \Delta_0, d_0)$-LIST-PHOM. \todo{\textsc{List $3$-Coloring}?}
%
%We start from fixing a few constants that will be needed later in the proof.
%Let $\alpha=O(1)$ be such that 
%\begin{equation}\label{eq:a}
%\Delta_0=\alpha(\log d_0)^{1/2} \, .
%\end{equation}
%Let $\beta=O(1)$ be a large enough constant such that
%\begin{equation}\label{eq:b}
%\beta > 4 \text{ and } 4 \alpha^2 \log{d_0}\cdot d_0^{2+16 \alpha^2} < d_0^\beta
%\end{equation}
%Finally, let $\gamma=O(1)$ be a small enough constant such that
%\begin{equation}\label{eq:g}
%c_0> 2^{\log^{\gamma}d_0} \text{ and } \sqrt{2} > \beta^\gamma \, .
%\end{equation}
%
%From the definition \eqref{eq:a} of $\alpha$ and definition (\ref{eq:g}) of $\gamma$ we know that there is no $2^{\sqrt{n}\log^{\gamma}d_0}$ algorithm for $(n, \alpha(\log d_0)^{1/2}, d_0)$-LIST-PHOM.
%Using a reduction from Lemma~\ref{lemma:red} one concludes that there are no
%$2^{\sqrt{n}\log^{\gamma}d_0}$ algorithm for 
%\begin{equation}\label{eq:longhom}
%(n/2, 2\alpha(\log d_0)^{1/2}, 4 \alpha^2 \log{d_0}\cdot d_0^{2+16 \alpha^2})\text{-LIST-PHOM} \, .
%\end{equation}
%
%Let now $n_1=n/2$ and $d_1=d_0^\beta$. It follows from the definition \eqref{eq:b} of $\beta$
%that
%\begin{equation}\label{eq:u}
%2\alpha(\log d_0)^{1/2} < \alpha (\log d_1)^{1/2} \, .
%\end{equation}
%
%From \eqref{eq:longhom} and \eqref{eq:u} it follows that there is no 
%$2^{\sqrt{n}\log^{\gamma}d_0}$ algorithm for $(n_1,\alpha(\log d_1)^{1/2}, d_1)$-LIST-PHOM.
%Finally, we note that there is no $2^{\sqrt{n_1}\log^{\gamma}d_1}$ for $(n_1,\alpha(\log d_1)^{1/2}, d_1)$-LIST-PHOM just because
%\[ 2^{\sqrt{n}\log^\gamma d_0}=2^{2\sqrt{n_1} \log^\gamma d_1/\beta^\gamma} > 2^{\sqrt{n_1}\log^\gamma d_1},\]
%where the last inequality follows from the definition \eqref{eq:g} of $\gamma$.
%
%By applying the same step we conclude that there is no $2^{\sqrt{n}\log^\gamma d}$ algorithm for $(n,d)$-LIST-PHOM for any large~$d$. Theorem~\ref{thm:homtolhom} then implies that such an algorithm is impossible also for $(n,d)$-PHOM.
%\end{proof}

==> proofs.tex <==
\noindent\usebox{\boxlemmathree}
\input{l3proof.tex}

\noindent\usebox{\boxlemmafour}
\input{l4proof.tex}

\noindent\usebox{\boxlemmafive}
\input{l5proof.tex}
